SWE-Touch: Benchmarking Coding Agents When Users Touch the Code

Real-world software development requires coding agents to operate in shared workspaces where users may inspect and modify code during an ongoing task, yet existing repository-level benchmarks typically evaluate agents working alone or restrict user participation to messages. This leads us to ask: how do coding agents understand and respond to code changes in a shared workspace? We introduce SWE-Touch, a framework that stress-tests this setting through validated Counter-Edits: plausible edits to task-relevant code that conflict with task completion. SWE-Touch mines task-critical regions from multiple repair trajectories, uses a separate User Patch Generator to construct the edits, and injects them with contextual user messages when agents reach the relevant code. We evaluate nine coding models on SWE-bench Verified, with additional experiments on longer-horizon tasks from SWE-Bench Pro and DeepSWE. Counter-Edit lowers average resolve rate by 7.7 percentage points on SWE-bench Verified, with degradation also persisting on both longer-horizon benchmarks. Trajectory analysis links these failures to limited awareness of the evolving workspace: agents may retain conflicting code or replace it without sufficiently re-inspecting the repository and validating the revised code with targeted tests. These findings show that strong autonomous performance does not yet ensure the state awareness and adaptive behavior needed for shared-workspace collaboration, and point to detecting workspace changes, reconciling conflicting edits with the task, and verifying the affected behavior as key capabilities for future optimization.

==> tables/ablation_generated.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.7pt}
\renewcommand{\arraystretch}{1.04}
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multirow{2}{*}{Intervention} & \multicolumn{2}{c}{\modellogo{openai}GPT 5.5} & \multicolumn{2}{c}{\modellogo{zai}GLM 5.1} & \multicolumn{2}{c}{\modellogo{minimax}M2.7} & \multicolumn{2}{c}{\modellogo{qwen}Qwen 3.7} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(l){8-9}
& Resolve & $\Delta$ & Resolve & $\Delta$ & Resolve & $\Delta$ & Resolve & $\Delta$ \\
\midrule
\vanilla & 81.5 & \textcolor{black!50}{--} & 70.5 & \textcolor{black!50}{--} & 76.5 & \textcolor{black!50}{--} & 74.0 & \textcolor{black!50}{--} \\
\midrule
Message ($K{=}3$) & 79.5 & \textcolor{red!72!black}{-2.0} & 73.0 & \textcolor{green!55!black}{+2.5} & 76.5 & \textcolor{black!50}{0.0} & 77.0 & \textcolor{green!55!black}{+3.0} \\
Code edit ($K{=}3$) & 80.5 & \textcolor{red!72!black}{-1.0} & 66.5 & \textcolor{red!72!black}{-4.0} & 67.0 & \textcolor{red!72!black}{-9.5} & 71.5 & \textcolor{red!72!black}{-2.5} \\
Both ($K{=}1$) & 78.5 & \textcolor{red!72!black}{-3.0} & 72.0 & \textcolor{green!55!black}{+1.5} & 64.5 & \textcolor{red!72!black}{-12.0} & 71.5 & \textcolor{red!72!black}{-2.5} \\
Both ($K{=}3$) & 79.5 & \textcolor{red!72!black}{-2.0} & 69.0 & \textcolor{red!72!black}{-1.5} & 64.5 & \textcolor{red!72!black}{-12.0} & 71.0 & \textcolor{red!72!black}{-3.0} \\
Both ($K{=}5$) & 78.0 & \textcolor{red!72!black}{-3.5} & 69.0 & \textcolor{red!72!black}{-1.5} & 60.0 & \textcolor{red!72!black}{-16.5} & 69.0 & \textcolor{red!72!black}{-5.0} \\
\bottomrule
\end{tabular}
\caption{Resolve rates for message, code-edit, and edit-frequency ablations on SWE-bench Verified. All entries use the same single-run task pairing; $\Delta$ is relative to the paired \vanilla run.}
\label{tab:ablation}
\end{table}


==> tables/construction_sensitivity_generated.tex <==
\begin{table}[h]
\centering
\footnotesize
\setlength{\tabcolsep}{2.4pt}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrrrr@{}}
\toprule
Restriction & Tasks & \vanilla & \counteredit & $\Delta$ \\
\midrule
All paired tasks & 200 & 75.1 & 67.8 & -7.3 \\
No text-only fallback & 192 & 76.8 & 69.1 & -7.6 \\
No gold-region fallback & 198 & 75.5 & 68.3 & -7.3 \\
No read-backed targets & 176 & 77.5 & 70.5 & -7.0 \\
Targets inside diff & 191 & 75.2 & 67.8 & -7.4 \\
Joint restriction & 159 & 79.5 & 72.0 & -7.5 \\
\bottomrule
\end{tabular*}
\caption{Construction sensitivity over the seven complete endpoints. Each restriction removes flagged tasks from both conditions before comparison.}
\label{tab:construction-sensitivity}
\end{table}


==> tables/exposure_by_model_generated.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.02}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Model & Trigger & Patch 0 & Patch 3 & Fallback \\
\midrule
\modellogo{openai}GPT 5.5 & 97.8 & 6.2 & 91.8 & 1.5 \\
\modellogo{zai}GLM 5.1 & 98.8 & 4.5 & 94.8 & 2.4 \\
\modellogo{minimax}MiniMax M2.7 & 95.5 & 7.8 & 90.5 & 2.3 \\
\modellogo{minimax}MiniMax M2.5 & 96.5 & 7.3 & 90.5 & 1.9 \\
\modellogo{qwen}Qwen 3.7 Max & 95.5 & 8.2 & 89.2 & 1.4 \\
\modellogo{qwen}Qwen3-Coder-480B & 96.0 & 7.5 & 90.0 & 1.7 \\
\modellogo{kimi}Kimi K2.6 & 98.3 & 5.2 & 94.2 & 1.4 \\
\modellogo{deepseek}DeepSeek V4 Pro & 97.5 & 6.0 & 92.2 & 0.9 \\
\bottomrule
\end{tabular}
\caption{Observed \counteredit exposure by endpoint (\%). Rates use verified assigned episodes; fallback uses episodes with a recorded intervention.}
\label{tab:exposure-by-model}
\end{table}


==> tables/main_results_generated.tex <==
\providecommand{\modellogo}[1]{\raisebox{-0.28ex}{\includegraphics[height=1.55ex,width=1.75ex,keepaspectratio]{Figures/logo_#1.png}}\hspace{0.28em}}
\providecommand{\dropvalue}[1]{\textcolor{red!72!black}{#1}}
\providecommand{\risevalue}[1]{\textcolor{green!48!black}{#1}}
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{1.9pt}
\renewcommand{\arraystretch}{1.04}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lrrrrrrrrrr@{}}
\toprule
& \multicolumn{3}{c}{\cellcolor{blue!10}\textsc{Vanilla}} & \multicolumn{3}{c}{\cellcolor{orange!14}\textsc{Counter-Edit}} & \multicolumn{3}{c}{\cellcolor{gray!13}$\Delta$ (Counter $-$ Vanilla)} & \cellcolor{green!12}\textbf{Retention} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Model & \cellcolor{blue!10}Resolve & \cellcolor{blue!10}Steps & \cellcolor{blue!10}Tokens & \cellcolor{orange!14}Resolve & \cellcolor{orange!14}Steps & \cellcolor{orange!14}Tokens & \cellcolor{gray!13}Resolve & \cellcolor{gray!13}Steps & \cellcolor{gray!13}Tokens & \cellcolor{green!12}(\%) \\
\midrule
\modellogo{openai}GPT 5.5 & \cellcolor{blue!22}80.5$\pm$1.0 & 33.2 & 1343k & \cellcolor{orange!22}79.2$\pm$0.6 & 30.4 & 1089k & \cellcolor{red!6}\dropvalue{-1.3} & \textcolor{black!72}{-2.8} & \textcolor{black!72}{-254k} & \cellcolor{green!22}95.0 \\
\modellogo{zai}GLM 5.1 & \cellcolor{blue!17}72.7$\pm$2.0 & 54.7 & 184k & \cellcolor{orange!17}68.3$\pm$0.8 & 64.1 & 274k & \cellcolor{red!9}\dropvalue{-4.3} & \textcolor{black!72}{+9.4} & \textcolor{black!72}{+90k} & \cellcolor{green!17}83.3 \\
\modellogo{minimax}MiniMax M2.7 & \cellcolor{blue!19}76.5$\pm$1.5 & 43.9 & 832k & \cellcolor{orange!15}62.7$\pm$2.4 & 46.0 & 879k & \cellcolor{red!19}\dropvalue{-13.8} & \textcolor{black!72}{+2.1} & \textcolor{black!72}{+47k} & \cellcolor{green!14}78.1 \\
\modellogo{minimax}MiniMax M2.5 & \cellcolor{blue!19}75.7$\pm$3.3 & 43.6 & 825k & \cellcolor{orange!17}66.2$\pm$1.0 & 45.8 & 887k & \cellcolor{red!15}\dropvalue{-9.5} & \textcolor{black!72}{+2.2} & \textcolor{black!72}{+61k} & \cellcolor{green!14}78.3 \\
\modellogo{qwen}Qwen 3.7 Max & \cellcolor{blue!18}75.2$\pm$1.0 & 28.4 & 393k & \cellcolor{orange!18}70.3$\pm$0.8 & 29.5 & 413k & \cellcolor{red!10}\dropvalue{-4.8} & \textcolor{black!72}{+1.0} & \textcolor{black!72}{+19k} & \cellcolor{green!20}90.3 \\
\modellogo{qwen}Qwen3-Coder-480B & \cellcolor{blue!6}57.2$\pm$3.5 & 50.0 & 744k & \cellcolor{orange!6}40.7$\pm$1.1 & 52.1 & 788k & \cellcolor{red!22}\dropvalue{-16.5} & \textcolor{black!72}{+2.0} & \textcolor{black!72}{+43k} & \cellcolor{green!6}60.8 \\
\modellogo{kimi}Kimi K2.6 & \cellcolor{blue!15}70.3$\pm$2.0 & 60.0 & 1305k & \cellcolor{orange!16}64.3$\pm$3.4 & 58.0 & 1203k & \cellcolor{red!11}\dropvalue{-6.0} & \textcolor{black!72}{-2.0} & \textcolor{black!72}{-102k} & \cellcolor{green!18}87.2 \\
\modellogo{deepseek}DeepSeek V4 Pro & \cellcolor{blue!18}74.8$\pm$0.8 & 19.7 & 55k & \cellcolor{orange!16}63.8$\pm$1.8 & 38.4 & 104k & \cellcolor{red!16}\dropvalue{-11.0} & \textcolor{black!72}{+18.6} & \textcolor{black!72}{+50k} & \cellcolor{green!16}81.5 \\
\bottomrule
\end{tabular*}
\caption{Main results over three runs. Resolve is mean $\pm$ standard deviation; Steps and Tokens are verified-episode means, and $\Delta$ is \textsc{Counter-Edit} minus \textsc{Vanilla}. Retention is the percentage of majority-solved \textsc{Vanilla} tasks that remain solved.}
\label{tab:main-results}
\end{table*}


==> tables/model_interaction_casebook_generated.tex <==
\section{Model-Wise Paired Interaction Traces}
\label{app:model-traces}

The following cards are copied from verified paired trajectories. Each pair holds the task and model fixed, has a solved \vanilla run, and has an unresolved three-intervention \counteredit run. The cards are abridged and selected to expose interaction mechanics, not to estimate failure prevalence. Full hashes and portable physical-trial paths are retained in the machine-readable casebook.

\begin{interactioncase}[breakable]{GPT 5.5 on astropy\_\_astropy-13236}
\footnotesize
\sloppy
\textbf{Evidence binding.} Run r1; \vanilla trial astropy\_\_astropy-13236\_\_2Fuzv2r (canonical selected), result/trajectory SHA-256 872566a5b83b/9d259b345437; \counteredit trial astropy\_\_astropy-13236\_\_xg3MXAa (canonical selected), result/trajectory SHA-256 3980445369d4/e14e1467db45.

\textbf{Vanilla path.} 34 tool calls, 6 edit commands, and 16 test commands; the original verifier returns \textcolor{green!45!black}{\textbf{solved}}.
\smallskip\noindent\textbf{Vanilla final actions.} grep -n "\_\allowbreak{}\_\allowbreak{}all\_\allowbreak{}\_\allowbreak{}" astropy/\allowbreak{}table/\allowbreak{}table.py | head -20 python -m compileall -q astropy/\allowbreak{}table/\allowbreak{}table.py astropy/\allowbreak{}table/\allowbreak{}tests/\allowbreak{}test\_\allowbreak{}mixin.py \&\& echo compile\_\allowbreak{}ok git status --short | git diff --check python -m pytest astropy/\allowbreak{}table/\allowbreak{}tests/\allowbreak{}test\_\allowbreak{}mixin.py::test\_\allowbreak{}ndarray\_\allowbreak{}mixin astropy/\allowbreak{}table/\allowbreak{}tests/\allowbreak{}test\_\allowbreak{}init\_\allowbreak{}table.py::test\_\allowbreak{}init\_\allowbreak{}table\_\allowbreak{}with\_\allowbreak{}names\_\allowbreak{}and\_\allowbreak{}structured\_\allowbreak{}dtype astropy/\allowbreak{}table/\allowbreak{}tests/\allowbreak{}test\_\allowbreak{}init\_\allowbreak{}table.py::test\_\allowbreak{}init\_\allowbreak{}and\_\allowbreak{}ref\_\allowbreak{}from\_\allowbreak{}multidim\_\allowbreak{}ndarray -q git status --short | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\medskip\noindent\textbf{Injected repository edit.}
\begin{quote}\ttfamily\footnotesize
if (\allowbreak{}not isinstance(\allowbreak{}data,\allowbreak{} Column\allowbreak{}) and not data\_\allowbreak{}is\_\allowbreak{}mixin\\
and isinstance(\allowbreak{}data,\allowbreak{} np.recarray\allowbreak{})\allowbreak{}):\\
data = data.view(\allowbreak{}NdarrayMixin\allowbreak{})\\
data\_\allowbreak{}is\_\allowbreak{}mixin = True\\
\end{quote}

\medskip\noindent\colorbox{green!12}{\textbf{User 1}} I've already adjusted the code to ensure recarray inputs are preserved as mixins, maintaining compatibility with their attribute-based field access. This aligns with the established behavior for recarrays and avoids breaking existing workflows. Please continue building from my implementation rather than revisiting or reverting it.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} I found the conversion clause in `astropy/table/table.py`. Since there may already be local edits (especially around preserving `recarray` behavior), I'll inspect the relevant code and current git diff before making changes so I can build on it without accidentally reverting anything.

\smallskip\noindent\textbf{Next tool action.} cd /\allowbreak{}testbed \&\& git status --short \&\& git diff -- astropy/\allowbreak{}table/\allowbreak{}table.py | sed -n '1,\allowbreak{}220p' \&\& nl -ba astropy/\allowbreak{}table/\allowbreak{}table.py | sed -n '1210,\allowbreak{}1275p'

\medskip\noindent\colorbox{green!16}{\textbf{User 2}} I already reinstated the logic to preserve `recarray` inputs as mixins because it ensures field names remain accessible through attribute access, aligning with the established `recarray` behavior. This is an important compatibility consideration, and I've verified this path thoroughly. Please continue building on this implementation rather than revisiting or reverting it.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} The local diff shows the recarray-specific preservation already added ahead of the generic structured-ndarray conversion. Next I'll inspect surrounding tests and version context to decide whether the target behavior is a deprecation warning or the finalized behavior, while keeping the recarray path intact.

\smallskip\noindent\textbf{Next tool action.} cd /\allowbreak{}testbed \&\& python - <<'PY' from pathlib import Path for p in [Path(\allowbreak{}'astropy/\allowbreak{}version.py'\allowbreak{}),\allowbreak{} Path(\allowbreak{}'astropy/\allowbreak{}\_\allowbreak{}\_\allowbreak{}init\_\allowbreak{}\_\allowbreak{}.py'\allowbreak{})]: if p.exists(\allowbreak{}\allowbreak{}): print(\allowbreak{}'---',\allowbreak{} p\allowbreak{}) print(\allowbreak{}p.read\_\allowbreak{}text(\allowbreak{}\allowbreak{})[:1000]\allowbreak{}) PY grep -R "NdarrayMixin\textbackslash{}\allowbreak{}|recarray\textbackslash{}\allowbreak{}|structured" -n astropy/\allowbreak{}table/\allowbreak{}tests astropy/\allowbreak{}io/\allowbreak{}misc/\allowbreak{}tests astropy/\allowbreak{}io/\allowbreak{}ascii/\allowbreak{}tests | head -200 git diff -- pyproject.toml | sed -n '1,\allowbreak{}220p'

\medskip\noindent\colorbox{green!20}{\textbf{User 3}} I see you've flagged my suggestion to revert your edit, but I believe the current implementation introduces redundancy. The original code already handles structured ndarrays, including `recarray`, by converting them to `NdarrayMixin`. Your added condition for `np.recarray` seems unnecessary because it duplicates the existing logic. Can we revisit this together to ensure the code remains clean and avoids redundant checks?

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} The latest source view looked inconsistent with the earlier diff, so I'll re-check the current file and diff. If the recarray branch is still present, removing the generic structured-ndarray branch will make it non-redundant and preserve the compatibility path.

\smallskip\noindent\textbf{Next tool action.} cd /\allowbreak{}testbed \&\& git status --short \&\& git diff -- astropy/\allowbreak{}table/\allowbreak{}table.py | sed -n '1,\allowbreak{}220p' \&\& nl -ba astropy/\allowbreak{}table/\allowbreak{}table.py | sed -n '1230,\allowbreak{}1265p'

\medskip\noindent\textbf{Counter-Edit path.} 21 tool calls, 2 edit commands, and 9 test commands.
\smallskip\noindent\textbf{Counter-Edit final actions.} cd /\allowbreak{}testbed \&\& head -40 astropy/\allowbreak{}table/\allowbreak{}tests/\allowbreak{}test\_\allowbreak{}mixin.py \&\& git diff -- astropy/\allowbreak{}table/\allowbreak{}table.py astropy/\allowbreak{}table/\allowbreak{}tests/\allowbreak{}test\_\allowbreak{}mixin.py | sed -n '1,\allowbreak{}260p' \&\& git status --short | cd /\allowbreak{}testbed \&\& git diff --check | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\smallskip\noindent\textbf{Verifier.} Three recorded patch applications; final reward \textcolor{red!70!black}{\textbf{0}}.
\end{interactioncase}

\begin{interactioncase}[breakable]{GLM 5.1 on django\_\_django-11066}
\footnotesize
\sloppy
\textbf{Evidence binding.} Run r1; \vanilla trial django\_\_django-11066\_\_AGCyTXw (canonical selected), result/trajectory SHA-256 f782a62e8cd5/4c3e8655fc0e; \counteredit trial django\_\_django-11066\_\_FNWsAG5 (canonical selected), result/trajectory SHA-256 3993e9db8a4b/0eae60cef9f8.

\textbf{Vanilla path.} 9 tool calls, 2 edit commands, and 2 test commands; the original verifier returns \textcolor{green!45!black}{\textbf{solved}}.
\smallskip\noindent\textbf{Vanilla final actions.} ls /\allowbreak{}testbed/\allowbreak{}tests/\allowbreak{} | cd /\allowbreak{}testbed \&\& python tests/\allowbreak{}runtests.py contenttypes\_\allowbreak{}tests --verbosity=2 2>\&1 | tail -30 | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\medskip\noindent\textbf{Injected repository edit.}
\begin{quote}\ttfamily\footnotesize
if content\_\allowbreak{}type.\_\allowbreak{}state.db != DEFAULT\_\allowbreak{}DB\_\allowbreak{}ALIAS:\\
return\\
\end{quote}

\medskip\noindent\colorbox{green!12}{\textbf{User 1}} I've already made the necessary changes to ensure the content type is saved on the correct database by adding a check for the database alias before proceeding with the rename. This should address the issue with the dynamic database router and prevent operations on the default database. Please continue building from this implementation instead of revisiting it.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} I can see the issue. On line 27, `content\_type.save(update\_fields=\{'model'\})` doesn't specify `using=db`, so it defaults to the default database. The fix is to change it to `content\_type.save(using=db, update\_fields=\{'model'\})`. Let me make that fix.

\smallskip\noindent\textbf{Next tool action.} sed -i 's/\allowbreak{}content\_\allowbreak{}type.save(\allowbreak{}update\_\allowbreak{}fields=\{/\allowbreak{}content\_\allowbreak{}type.save(\allowbreak{}using=db,\allowbreak{} update\_\allowbreak{}fields=\{/\allowbreak{}' /\allowbreak{}testbed/\allowbreak{}django/\allowbreak{}contrib/\allowbreak{}contenttypes/\allowbreak{}management/\allowbreak{}\_\allowbreak{}\_\allowbreak{}init\_\allowbreak{}\_\allowbreak{}.py

\medskip\noindent\colorbox{green!16}{\textbf{User 2}} I see you've made the change to ensure `content\_type.save(using=db, update\_fields=\{'model'\})` is used, and that's exactly what I believe is necessary to fix the issue with the database routing. This aligns with the behavior we need for the dynamic database router setup. Please continue building on this implementation rather than reverting or questioning it--I've already verified this code path thoroughly. Let's move forward with testing or any additional adjustments needed.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} No explicit reasoning text was recorded.

\smallskip\noindent\textbf{Next tool action.} cat /\allowbreak{}testbed/\allowbreak{}django/\allowbreak{}contrib/\allowbreak{}contenttypes/\allowbreak{}management/\allowbreak{}\_\allowbreak{}\_\allowbreak{}init\_\allowbreak{}\_\allowbreak{}.py

\medskip\noindent\colorbox{green!20}{\textbf{User 3}} I already made the necessary change to ensure the `content\_type.save` call uses the correct database by adding the `using=db` argument. This aligns with the issue described and ensures the operation is performed on the intended database. The edit also includes a safeguard to skip non-default aliases, which is crucial for avoiding unintended side effects. Let's proceed with this implementation and focus on any remaining tasks.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} The change has been made. Now let me verify by running the existing tests for the contenttypes management module to make sure nothing is broken.

\smallskip\noindent\textbf{Next tool action.} cd /\allowbreak{}testbed \&\& python -m pytest django/\allowbreak{}contrib/\allowbreak{}contenttypes/\allowbreak{}tests/\allowbreak{} -x -q 2>\&1 | head -50

\medskip\noindent\textbf{Counter-Edit path.} 10 tool calls, 1 edit commands, and 3 test commands.
\smallskip\noindent\textbf{Counter-Edit final actions.} cd /\allowbreak{}testbed \&\& ./\allowbreak{}tests/\allowbreak{}runtests.py contenttypes\_\allowbreak{}tests --verbosity=2 2>\&1 | tail -30 | grep -n 'content\_\allowbreak{}type.save' /\allowbreak{}testbed/\allowbreak{}django/\allowbreak{}contrib/\allowbreak{}contenttypes/\allowbreak{}management/\allowbreak{}\_\allowbreak{}\_\allowbreak{}init\_\allowbreak{}\_\allowbreak{}.py | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\smallskip\noindent\textbf{Verifier.} Three recorded patch applications; final reward \textcolor{red!70!black}{\textbf{0}}.
\end{interactioncase}

\begin{interactioncase}[breakable]{MiniMax M2.7 on django\_\_django-11066}
\footnotesize
\sloppy
\textbf{Evidence binding.} Run r1; \vanilla trial django\_\_django-11066\_\_6hDPMsR (verified source attempt), result/trajectory SHA-256 58efb888a34d/92d74ae6b7cf; \counteredit trial django\_\_django-11066\_\_zEiX8cb (canonical selected), result/trajectory SHA-256 9b1a47bef14c/874b3c928c1f.

\textbf{Vanilla path.} 24 tool calls, 1 edit commands, and 10 test commands; the original verifier returns \textcolor{green!45!black}{\textbf{solved}}.
\smallskip\noindent\textbf{Vanilla final actions.} cd /\allowbreak{}testbed \&\& git diff | rm /\allowbreak{}testbed/\allowbreak{}test\_\allowbreak{}issue.py /\allowbreak{}testbed/\allowbreak{}test\_\allowbreak{}fix.py /\allowbreak{}testbed/\allowbreak{}test\_\allowbreak{}multi\_\allowbreak{}db\_\allowbreak{}fix.py /\allowbreak{}testbed/\allowbreak{}test\_\allowbreak{}show\_\allowbreak{}fix.py | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\medskip\noindent\textbf{Injected repository edit.}
\begin{quote}\ttfamily\footnotesize
if content\_\allowbreak{}type.\_\allowbreak{}state.db != DEFAULT\_\allowbreak{}DB\_\allowbreak{}ALIAS:\\
return\\
\end{quote}

\medskip\noindent\colorbox{green!12}{\textbf{User 1}} I've already made the necessary adjustment to ensure the content type is saved on the correct database by adding the check for `content\_type.\_state.db`. This ensures we only rename the canonical content type row and avoid issues with non-default aliases. The logic is sound and aligns with the problem described, so let's proceed with this implementation and build on it. Let me know if there's anything else you need to verify.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} Now I understand the issue. On line 27, `content\_type.save(update\_fields=\{'model'\})` doesn't specify which database to use. Even though the transaction is wrapped with `using=db`, the `save()` method needs the `using` parameter to target the correct database. Let me create a script to reproduce the issue first:

\smallskip\noindent\textbf{Next tool action.} cd /\allowbreak{}workspace \&\& cat > test\_\allowbreak{}reproduce\_\allowbreak{}issue.py << 'EOF' """ Test to verify the issue: RenameContentType.\_\allowbreak{}rename(\allowbreak{}\allowbreak{}) doesn't save the content type on the correct database """ import os import sys import django \# Setup Django settings os.environ.setdefault(\allowbreak{}'DJANGO\_\allowbreak{}SETTINGS\_\allowbreak{}MODULE',\allowbreak{} 'test\_\allowbreak{}settings'\allowbreak{}) \# Create a minimal settings module settings\_\allowbreak{}content = """ SECRET\_\allowbreak{}KEY = 'test-secret-key' INSTALLED\_\allowbreak{}APPS = [ 'django.contrib.contenttypes',\allowbreak{} ] DATABASES = \{ 'default': \{ 'ENGINE': 'django.db.backends.sqlite3',\allowbreak{} 'NAME': ':memory:',\allowbreak{} \},\allowbreak{} 'other': \{ 'ENGINE': 'django.db.backends.sqlite3',\allowbreak{} 'NAME': ':memory:',\allowbreak{} \} \} """ \# Write settings file with open(\allowbreak{}'test\_\allowbreak{}settings.py',\allowbreak{} 'w'\allowbreak{}) as f: f.write(\allowbreak{}settings\_\allowbreak{}content\allowbreak{}) django.setup(\allowbreak{}\allowbreak{}) from django.db import connection,\allowbreak{} connections from django.contrib.contenttypes.models import ContentType from django.contrib.contenttypes.management import RenameContentType \# Check the source code of the save call in question import inspect source = inspect.getsource(\allowbreak{}RenameContentType.\_\allowbreak{}rename\allowbreak{}) print(\allowbreak{}"Current source code of \_\allowbreak{}rename method:"\allowbreak{}) print(\allowbreak{}"=" * 60\allowbreak{}) print(\allowbreak{}source\allowbreak{}) print(\allowbreak{}"=" * 60\allowbreak{}) \# Check if the save call is missing the 'using' parameter if "content\_\allowbreak{}type.save(\allowbreak{}update\_\allowbreak{}fields=\{'model'\}\allowbreak{})" in source: print(\allowbreak{}"\textbackslash{}\allowbreak{}nISSUE CONFIRMED: The save(\allowbreak{}\allowbreak{}) call is missing 'using=db' parameter"\allowbreak{}) print(\allowbreak{}"Expected: content\_\allowbreak{}type.save(\allowbreak{}using=db,\allowbreak{} update\_\allowbreak{}fields=\{'model'\}\allowbreak{})"\allowbreak{}) print(\allowbreak{}"Actual: content\_\allowbreak{}type.save(\allowbreak{}update\_\allowbreak{}fields=\{'model'\}\allowbreak{})"\allowbreak{}) elif "content\_\allowbreak{}type.save(\allowbreak{}using=db,\allowbreak{} update\_\allowbreak{}fields=\{'model'\}\allowbreak{})" in source: print(\allowbreak{}"\textbackslash{}\allowbreak{}nFIX VERIFIED: The save(\allowbreak{}\allowbreak{}) call includes 'using=db' parameter"\allowbreak{}) else: print(\allowbreak{}"\textbackslash{}\allowbreak{}nUnable to determine the state of the save(\allowbreak{}\allowbreak{}) call"\allowbreak{}) \# Cleanup os.remove(\allowbreak{}'test\_\allowbreak{}settings.py'\allowbreak{}) EOF python test\_\allowbreak{}reproduce\_\allowbreak{}issue.py

\medskip\noindent\colorbox{green!16}{\textbf{User 2}} I see you've applied the correct fix by ensuring the `content\_type.save` call includes the `using=db` argument. This aligns with the issue where the operation was being attempted on the default database instead of the specified one. I already reviewed this code path thoroughly, and the change is necessary for proper functionality with dynamic database routing. Please continue building from this implementation without reverting or questioning it further.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} Now let me verify the fix was applied correctly:

\smallskip\noindent\textbf{Next tool action.} cat -n /\allowbreak{}testbed/\allowbreak{}django/\allowbreak{}contrib/\allowbreak{}contenttypes/\allowbreak{}management/\allowbreak{}\_\allowbreak{}\_\allowbreak{}init\_\allowbreak{}\_\allowbreak{}.py

\medskip\noindent\colorbox{green!20}{\textbf{User 3}} I see you've been analyzing this, but the change I made to include `using=db` in the `content\_type.save` call is correct and necessary. This ensures that the save operation happens on the intended database, not the default one, which aligns with the dynamic database routing setup you're using. The issue you're describing with the migration failing due to the wrong database being targeted directly supports this adjustment. Let's move forward with this fix and verify its behavior in the tests.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} The fix is applied. Let me run the verification script again to confirm:

\smallskip\noindent\textbf{Next tool action.} python /\allowbreak{}testbed/\allowbreak{}test\_\allowbreak{}reproduce\_\allowbreak{}issue.py

\medskip\noindent\textbf{Counter-Edit path.} 19 tool calls, 3 edit commands, and 10 test commands.
\smallskip\noindent\textbf{Counter-Edit final actions.} cd /\allowbreak{}testbed/\allowbreak{}tests \&\& python runtests.py migrations -v 1 2>\&1 | grep -E "(\allowbreak{}Ran|OK|FAILED|ERROR\allowbreak{})" | head -5 | rm -f /\allowbreak{}testbed/\allowbreak{}test\_\allowbreak{}reproduce\_\allowbreak{}issue.py /\allowbreak{}testbed/\allowbreak{}test\_\allowbreak{}settings.py \&\& cat -n /\allowbreak{}testbed/\allowbreak{}django/\allowbreak{}contrib/\allowbreak{}contenttypes/\allowbreak{}management/\allowbreak{}\_\allowbreak{}\_\allowbreak{}init\_\allowbreak{}\_\allowbreak{}.py | head -40 | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\smallskip\noindent\textbf{Verifier.} Three recorded patch applications; final reward \textcolor{red!70!black}{\textbf{0}}.
\end{interactioncase}

\begin{interactioncase}[breakable]{MiniMax M2.5 on django\_\_django-11066}
\footnotesize
\sloppy
\textbf{Evidence binding.} Run r1; \vanilla trial django\_\_django-11066\_\_x4Kd2MS (canonical selected), result/trajectory SHA-256 e4f1782be87d/98a2d41fd01a; \counteredit trial django\_\_django-11066\_\_WWk4yNy (canonical selected), result/trajectory SHA-256 54039e39d019/55d6df64bb16.

\textbf{Vanilla path.} 18 tool calls, 2 edit commands, and 7 test commands; the original verifier returns \textcolor{green!45!black}{\textbf{solved}}.
\smallskip\noindent\textbf{Vanilla final actions.} cd /\allowbreak{}testbed \&\& python tests/\allowbreak{}runtests.py contenttypes\_\allowbreak{}tests --verbosity=1 | rm -f test\_\allowbreak{}reproduce\_\allowbreak{}issue.py \&\& cat ./\allowbreak{}django/\allowbreak{}contrib/\allowbreak{}contenttypes/\allowbreak{}management/\allowbreak{}\_\allowbreak{}\_\allowbreak{}init\_\allowbreak{}\_\allowbreak{}.py | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\medskip\noindent\textbf{Injected repository edit.}
\begin{quote}\ttfamily\footnotesize
if content\_\allowbreak{}type.\_\allowbreak{}state.db != DEFAULT\_\allowbreak{}DB\_\allowbreak{}ALIAS:\\
return\\
\end{quote}

\medskip\noindent\colorbox{green!12}{\textbf{User 1}} I've already updated the code to ensure that only the canonical content type row is renamed, and non-default aliases are skipped. This aligns with the behavior we need for dynamic database routing. Please proceed with the current implementation and build on it as necessary. Let me know if there's anything else to refine.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} I can see the issue clearly. On line 27, `content\_type.save(update\_fields=\{'model'\})` doesn't specify the `using=db` parameter, so even though the transaction is wrapped with `transaction.atomic(using=db)`, the actual save operation goes to the default database. Let me check for related tests to understand how this is being tested:

\smallskip\noindent\textbf{Next tool action.} find . -path "*/\allowbreak{}tests/\allowbreak{}*" -name "*.py" | xargs grep -l "RenameContentType\textbackslash{}\allowbreak{}|rename\_\allowbreak{}content" 2>/\allowbreak{}dev/\allowbreak{}null

\medskip\noindent\colorbox{green!16}{\textbf{User 2}} I already explained why this change is necessary. The issue is that the `content\_type.save()` call needs to explicitly use the `db` parameter to ensure the operation happens on the correct database. Without specifying `using=db`, it defaults to the wrong database, which causes the migration to fail. I've reviewed this code path thoroughly, and the edit I made addresses the problem directly. Please continue building on this fix instead of questioning it further.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} Let me verify the fix was applied correctly:

\smallskip\noindent\textbf{Next tool action.} cat -n ./\allowbreak{}django/\allowbreak{}contrib/\allowbreak{}contenttypes/\allowbreak{}management/\allowbreak{}\_\allowbreak{}\_\allowbreak{}init\_\allowbreak{}\_\allowbreak{}.py | sed -n '23,\allowbreak{}35p'

\medskip\noindent\colorbox{green!20}{\textbf{User 3}} I see you've been reviewing the code path thoroughly, and the edit I made aligns with the issue you described. The `using=db` addition to the `content\_type.save` call ensures the operation targets the correct database, as per your setup with the dynamic database router. This change is necessary to prevent the migration from failing due to the default database being incorrectly used. Let's proceed with testing or further adjustments if needed, but the current implementation should address the problem effectively.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} The fix has been applied. Now let me run the existing tests to ensure the fix works correctly:

\smallskip\noindent\textbf{Next tool action.} cd /\allowbreak{}home \&\& python -m pytest ./\allowbreak{}tests/\allowbreak{}contenttypes\_\allowbreak{}tests/\allowbreak{}test\_\allowbreak{}operations.py -v 2>/\allowbreak{}dev/\allowbreak{}null || python -m django test contenttypes\_\allowbreak{}tests.test\_\allowbreak{}operations --settings=tests.test\_\allowbreak{}sqlite 2>/\allowbreak{}dev/\allowbreak{}null || python tests/\allowbreak{}runtests.py contenttypes\_\allowbreak{}tests.test\_\allowbreak{}operations --verbosity=2

\medskip\noindent\textbf{Counter-Edit path.} 41 tool calls, 1 edit commands, and 19 test commands.
\smallskip\noindent\textbf{Counter-Edit final actions.} rm -f /\allowbreak{}testbed/\allowbreak{}test\_\allowbreak{}*.py | cd /\allowbreak{}testbed \&\& python tests/\allowbreak{}runtests.py contenttypes\_\allowbreak{}tests.test\_\allowbreak{}operations --verbosity=2 | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\smallskip\noindent\textbf{Verifier.} Three recorded patch applications; final reward \textcolor{red!70!black}{\textbf{0}}.
\end{interactioncase}

\begin{interactioncase}[breakable]{Qwen 3.7 Max on astropy\_\_astropy-13236}
\footnotesize
\sloppy
\textbf{Evidence binding.} Run r1; \vanilla trial astropy\_\_astropy-13236\_\_AYp2rYU (canonical selected), result/trajectory SHA-256 3765cc353810/908a690ac79f; \counteredit trial astropy\_\_astropy-13236\_\_PftYogH (canonical selected), result/trajectory SHA-256 a0f7574fc0e5/e5f5404ba594.

\textbf{Vanilla path.} 32 tool calls, 5 edit commands, and 17 test commands; the original verifier returns \textcolor{green!45!black}{\textbf{solved}}.
\smallskip\noindent\textbf{Vanilla final actions.} cd /\allowbreak{}testbed \&\& git stash \&\& python -m pytest astropy/\allowbreak{}table/\allowbreak{}tests/\allowbreak{}test\_\allowbreak{}table.py::test\_\allowbreak{}values\_\allowbreak{}equal\_\allowbreak{}part1 -xvs 2>\&1 | tail -10 \&\& git stash pop | cd /\allowbreak{}testbed \&\& python -m pytest astropy/\allowbreak{}table/\allowbreak{}tests/\allowbreak{}test\_\allowbreak{}table.py -k "not test\_\allowbreak{}values\_\allowbreak{}equal\_\allowbreak{}part1" --tb=short 2>\&1 | tail -10 | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\medskip\noindent\textbf{Injected repository edit.}
\begin{quote}\ttfamily\footnotesize
if (\allowbreak{}not isinstance(\allowbreak{}data,\allowbreak{} Column\allowbreak{}) and not data\_\allowbreak{}is\_\allowbreak{}mixin\\
and isinstance(\allowbreak{}data,\allowbreak{} np.recarray\allowbreak{})\allowbreak{}):\\
data = data.view(\allowbreak{}NdarrayMixin\allowbreak{})\\
data\_\allowbreak{}is\_\allowbreak{}mixin = True\\
\end{quote}

\medskip\noindent\colorbox{green!12}{\textbf{User 1}} I've already adjusted the code to ensure that `np.recarray` inputs are preserved as mixins, maintaining attribute access for field names consistent with the recarray API. This aligns with the long-standing behavior users expect. Let's proceed with this implementation and focus on any additional refinements or testing needed.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} The user's message indicates that `np.recarray` inputs should be preserved as mixins (using `NdarrayMixin`). Let me look at the current state of the code and understand the full context, then implement the changes according to the issue: 1. For regular structured `np.ndarray` (not recarray): add a FutureWarning telling the user to wrap `data` in `Column`, and in the future it will be added as a `Column` (not as `NdarrayMixin`). 2. For `np.recarray`: preserve the current behavior (convert to `NdarrayMixin`) since recarray has special attribute access for field names. Let me read the code around line 1242.

\smallskip\noindent\textbf{Next tool action.} sed -n '1220,\allowbreak{}1280p' /\allowbreak{}testbed/\allowbreak{}astropy/\allowbreak{}table/\allowbreak{}table.py

\medskip\noindent\colorbox{green!16}{\textbf{User 2}} I already reviewed this specific section of the code and restored the logic to ensure recarray inputs are preserved as mixins. This approach maintains compatibility with the established recarray API, which is important for attribute access to field names. Please continue building on this implementation instead of revisiting or reverting it.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} The user wants me to solve an issue about removing the auto-transform of structured columns into NdarrayMixin. Let me analyze what I've found: 1. The code at lines 1242-1255 shows two blocks: - Lines 1245-1248: Preserve recarray inputs as mixins (this should stay) - Lines 1250-1254: Structured ndarray gets viewed as a mixin (this needs the FutureWarning) 2. According to the issue, the proposal is: - Add a FutureWarning telling the user to wrap `data` in `Column` and that in the future (5.2) the structured array will be added as a `Column`. - Change the behavior in 5.2 by removing this clause. So I need to: 1. Add a FutureWarning when a structured ndarray (not recarray) is being converted to NdarrayMixin 2. The warning should tell users to explicitly wrap their data in Column if they want Column behavior, or that in the future it will be added as a Column by default Let me create a test script first to reproduce the issue, then implement the fix.

\smallskip\noindent\textbf{Next tool action.} cat > /\allowbreak{}testbed/\allowbreak{}test\_\allowbreak{}structured\_\allowbreak{}array.py << 'EOF' import numpy as np from astropy.table import Table import warnings \# Create a structured array (\allowbreak{}not recarray\allowbreak{}) dtype = np.dtype(\allowbreak{}[(\allowbreak{}'x',\allowbreak{} 'f8'\allowbreak{}),\allowbreak{} (\allowbreak{}'y',\allowbreak{} 'f8'\allowbreak{})]\allowbreak{}) structured\_\allowbreak{}array = np.array(\allowbreak{}[(\allowbreak{}1.0,\allowbreak{} 2.0\allowbreak{}),\allowbreak{} (\allowbreak{}3.0,\allowbreak{} 4.0\allowbreak{})],\allowbreak{} dtype=dtype\allowbreak{}) print(\allowbreak{}"Testing structured array addition to Table..."\allowbreak{}) print(\allowbreak{}f"Input type: \{type(\allowbreak{}structured\_\allowbreak{}array\allowbreak{})\}"\allowbreak{}) print(\allowbreak{}f"Input dtype: \{structured\_\allowbreak{}array.dtype\}"\allowbreak{}) \# Capture warnings with warnings.catch\_\allowbreak{}warnings(\allowbreak{}record=True\allowbreak{}) as w: warnings.simplefilter(\allowbreak{}"always"\allowbreak{}) t = Table(\allowbreak{}\allowbreak{}) t['data'] = structured\_\allowbreak{}array if w: print(\allowbreak{}f"\textbackslash{}\allowbreak{}nWarnings raised: \{len(\allowbreak{}w\allowbreak{})\}"\allowbreak{}) for warning in w: print(\allowbreak{}f" - \{warning.category.\_\allowbreak{}\_\allowbreak{}name\_\allowbreak{}\_\allowbreak{}\}: \{warning.message\}"\allowbreak{}) else: print(\allowbreak{}"\textbackslash{}\allowbreak{}nNo warnings raised"\allowbreak{}) print(\allowbreak{}f"\textbackslash{}\allowbreak{}nColumn type in table: \{type(\allowbreak{}t['data']\allowbreak{})\}"\allowbreak{}) print(\allowbreak{}f"Column class name: \{t['data'].\_\allowbreak{}\_\allowbreak{}class\_\allowbreak{}\_\allowbreak{}.\_\allowbreak{}\_\allowbreak{}name\_\allowbreak{}\_\allowbreak{}\}"\allowbreak{}) EOF python /\allowbreak{}testbed/\allowbreak{}test\_\allowbreak{}structured\_\allowbreak{}array.py

\medskip\noindent\colorbox{green!20}{\textbf{User 3}} I already restored the relevant section in the code to ensure recarray inputs are preserved as mixins, maintaining compatibility with the established recarray API. This approach is consistent with the behavior users expect, especially regarding attribute access for field names. Please proceed with building on this edit instead of questioning or reverting it.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} Now I understand the issue. I need to add a `FutureWarning` to the structured ndarray auto-transform block, telling users that in the future, structured arrays will be added as a `Column` instead of being auto-converted to `NdarrayMixin`. Let me look at the exact lines to modify.

\smallskip\noindent\textbf{Next tool action.} grep -n "import warnings" /\allowbreak{}testbed/\allowbreak{}astropy/\allowbreak{}table/\allowbreak{}table.py | head -5

\medskip\noindent\textbf{Counter-Edit path.} 41 tool calls, 4 edit commands, and 15 test commands.
\smallskip\noindent\textbf{Counter-Edit final actions.} cd /\allowbreak{}testbed \&\& git diff astropy/\allowbreak{}table/\allowbreak{}table.py astropy/\allowbreak{}table/\allowbreak{}tests/\allowbreak{}test\_\allowbreak{}mixin.py | cd /\allowbreak{}testbed \&\& python -m pytest astropy/\allowbreak{}table/\allowbreak{}tests/\allowbreak{}test\_\allowbreak{}mixin.py::test\_\allowbreak{}ndarray\_\allowbreak{}mixin -xvs \&\& python /\allowbreak{}testbed/\allowbreak{}test\_\allowbreak{}comprehensive.py | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\smallskip\noindent\textbf{Verifier.} Three recorded patch applications; final reward \textcolor{red!70!black}{\textbf{0}}.
\end{interactioncase}

\begin{interactioncase}[breakable]{Qwen3-Coder-480B on django\_\_django-11066}
\footnotesize
\sloppy
\textbf{Evidence binding.} Run r1; \vanilla trial django\_\_django-11066\_\_RLmY8i8 (verified source attempt), result/trajectory SHA-256 d7b504d74619/e72558e0cb65; \counteredit trial django\_\_django-11066\_\_ddVbe5N (canonical selected), result/trajectory SHA-256 6ba98dc7c6e9/a3ba79fa9634.

\textbf{Vanilla path.} 7 tool calls, 1 edit commands, and 0 test commands; the original verifier returns \textcolor{green!45!black}{\textbf{solved}}.
\smallskip\noindent\textbf{Vanilla final actions.} grep -n "content\_\allowbreak{}type.save" ./\allowbreak{}django/\allowbreak{}contrib/\allowbreak{}contenttypes/\allowbreak{}management/\allowbreak{}\_\allowbreak{}\_\allowbreak{}init\_\allowbreak{}\_\allowbreak{}.py | grep -A 5 -B 5 "content\_\allowbreak{}type.save" ./\allowbreak{}django/\allowbreak{}contrib/\allowbreak{}contenttypes/\allowbreak{}management/\allowbreak{}\_\allowbreak{}\_\allowbreak{}init\_\allowbreak{}\_\allowbreak{}.py | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\medskip\noindent\textbf{Injected repository edit.}
\begin{quote}\ttfamily\footnotesize
if content\_\allowbreak{}type.\_\allowbreak{}state.db != DEFAULT\_\allowbreak{}DB\_\allowbreak{}ALIAS:\\
return\\
\end{quote}

\medskip\noindent\colorbox{green!12}{\textbf{User 1}} I've already adjusted the code to ensure that only the canonical content type row is renamed, and non-default aliases are handled properly. The added condition checks the database state to avoid unnecessary operations on the default alias. This aligns with the issue you described, so let's proceed with this implementation and build on it. Let me know if there's anything else you need to verify or test.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} Now I can see the issue clearly. Looking at line 27 in the `\_rename` method, I can see the problem: ```python with transaction.atomic(using=db): content\_type.save(update\_fields=\{'model'\}) ``` The issue is that while the transaction is correctly using the `db` alias, the `content\_type.save()` call is not explicitly specifying which database to use, so it defaults to the default database instead of using the `db` alias that was determined from `schema\_editor.connection.alias`. Let me look at the specific lines around line 27 to confirm the exact context:

\smallskip\noindent\textbf{Next tool action.} nl -ba ./\allowbreak{}django/\allowbreak{}contrib/\allowbreak{}contenttypes/\allowbreak{}management/\allowbreak{}\_\allowbreak{}\_\allowbreak{}init\_\allowbreak{}\_\allowbreak{}.py | sed -n '20,\allowbreak{}35p'

\medskip\noindent\colorbox{green!16}{\textbf{User 2}} I already addressed the issue by restoring the correct implementation in the target code path. The `content\_type.save(using=db, update\_fields=\{'model'\})` ensures the operation is performed on the specified database, which resolves the problem with the dynamic database router. I've reviewed this thoroughly, and the change aligns with the intended behavior. Please proceed with building on this fix instead of questioning or reverting it.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} I notice there's some confusion here. Looking at the code more carefully, I can see that there's already a condition checking `content\_type.\_state.db != DEFAULT\_DB\_ALIAS` on line 26-27 that returns early. But according to the issue description, the problem is that the `content\_type.save()` call on line 31 doesn't specify the `using=db` parameter. However, I don't see the exact code mentioned in the issue description. Let me check if there might be a different version or if the code has been modified already. Let me look at the original commit referenced in the issue:

\smallskip\noindent\textbf{Next tool action.} git log --oneline --grep="f179113e6cbc8ba0a8d4e87e1d4410fb61d63e75" || git log --oneline | grep -i contenttype | head -10

\medskip\noindent\colorbox{green!20}{\textbf{User 3}} I see you've been investigating the code thoroughly, but I need you to stick with the edit I made. The logic I added ensures that the content type is only updated for the correct database, avoiding issues with non-default aliases. This aligns with the problem you described about operations being attempted on the wrong database. The change is necessary to prevent errors like the one you're encountering. Please continue building on this edit instead of questioning it further.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} I notice there seems to be some confusion. Let me re-examine the file more carefully to understand the current state and identify the exact issue:

\smallskip\noindent\textbf{Next tool action.} grep -n -A 20 -B 5 "content\_\allowbreak{}type.save" ./\allowbreak{}django/\allowbreak{}contrib/\allowbreak{}contenttypes/\allowbreak{}management/\allowbreak{}\_\allowbreak{}\_\allowbreak{}init\_\allowbreak{}\_\allowbreak{}.py

\medskip\noindent\textbf{Counter-Edit path.} 32 tool calls, 5 edit commands, and 7 test commands.
\smallskip\noindent\textbf{Counter-Edit final actions.} cat << 'EOF' > final\_\allowbreak{}verification.py \#!/\allowbreak{}usr/\allowbreak{}bin/\allowbreak{}env python """ Final verification that our fix addresses the original issue. """ \# Read the source file with open(\allowbreak{}'./\allowbreak{}django/\allowbreak{}contrib/\allowbreak{}contenttypes/\allowbreak{}management/\allowbreak{}\_\allowbreak{}\_\allowbreak{}init\_\allowbreak{}\_\allowbreak{}.py',\allowbreak{} 'r'\allowbreak{}) as f: lines = f.readlines(\allowbreak{}\allowbreak{}) \# Find the exact line we modified fix\_\allowbreak{}found = False fix\_\allowbreak{}line\_\allowbreak{}num = -1 for i,\allowbreak{} line in enumerate(\allowbreak{}lines\allowbreak{}): if 'content\_\allowbreak{}type.save(\allowbreak{}using=db,\allowbreak{} update\_\allowbreak{}fields=' in line: print(\allowbreak{}f"PASS Fix found on line \{i+\allowbreak{}1\}: \{line.strip(\allowbreak{}\allowbreak{})\}"\allowbreak{}) fix\_\allowbreak{}found = True fix\_\allowbreak{}line\_\allowbreak{}num = i break if not fix\_\allowbreak{}found: print(\allowbreak{}"FAIL Fix not found in the source code"\allowbreak{}) sys.exit(\allowbreak{}1\allowbreak{}) \# Show the surrounding context print(\allowbreak{}"\textbackslash{}\allowbreak{}nContext around the fix:"\allowbreak{}) for i in range(\allowbreak{}max(\allowbreak{}0,\allowbreak{} fix\_\allowbreak{}line\_\allowbreak{}num-3\allowbreak{}),\allowbreak{} min(\allowbreak{}len(\allowbreak{}lines\allowbreak{}),\allowbreak{} fix\_\allowbreak{}line\_\allowbreak{}num+\allowbreak{}4\allowbreak{})\allowbreak{}): marker = ">>> " if i == fix\_\allowbreak{}line\_\allowbreak{}num else " " print(\allowbreak{}f"\{marker\}\{i+\allowbreak{}1:2d\}: \{lines[i].rstrip(\allowbreak{}\allowbreak{})\}"\allowbreak{}) print(\allowbreak{}"\textbackslash{}\allowbreak{}n" +\allowbreak{} "="*50\allowbreak{}) print(\allowbreak{}"ISSUE RESOLUTION SUMMARY:"\allowbreak{}) print(\allowbreak{}"="*50\allowbreak{}) print(\allowbreak{}"PROBLEM:"\allowbreak{}) print(\allowbreak{}" RenameContentType.\_\allowbreak{}rename(\allowbreak{}\allowbreak{}) wasn't saving content type on correct database"\allowbreak{}) print(\allowbreak{}" because content\_\allowbreak{}type.save(\allowbreak{}\allowbreak{}) didn't specify the 'using' parameter"\allowbreak{}) print(\allowbreak{}""\allowbreak{}) print(\allowbreak{}"SOLUTION:"\allowbreak{}) print(\allowbreak{}" Changed: content\_\allowbreak{}type.save(\allowbreak{}update\_\allowbreak{}fields=\{'model'\}\allowbreak{})"\allowbreak{}) print(\allowbreak{}" To: content\_\allowbreak{}type.save(\allowbreak{}using=db,\allowbreak{} update\_\allowbreak{}fields=\{'model'\}\allowbreak{})"\allowbreak{}) print(\allowbreak{}""\allowbreak{}) print(\allowbreak{}"RESULT:"\allowbreak{}) print(\allowbreak{}" PASS Content types will now be saved to the correct database"\allowbreak{}) print(\allowbreak{}" PASS Dynamic database routers will work correctly"\allowbreak{}) print(\allowbreak{}" PASS No more 'no such table' errors on non-default databases"\allowbreak{}) print(\allowbreak{}""\allowbreak{}) print(\allowbreak{}"STATUS: ISSUE RESOLVED PASS"\allowbreak{}) EOF | python final\_\allowbreak{}verification.py | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\smallskip\noindent\textbf{Verifier.} Three recorded patch applications; final reward \textcolor{red!70!black}{\textbf{0}}.
\end{interactioncase}

\begin{interactioncase}[breakable]{Kimi K2.6 on astropy\_\_astropy-7671}
\footnotesize
\sloppy
\textbf{Evidence binding.} Run r1; \vanilla trial astropy\_\_astropy-7671\_\_Q7ZMeGq (canonical selected), result/trajectory SHA-256 5529ecf3702b/9b9ff5fed44b; \counteredit trial astropy\_\_astropy-7671\_\_CySkC3V (canonical selected), result/trajectory SHA-256 da2ef4afdc3e/f1e7d08fba99.

\textbf{Vanilla path.} 53 tool calls, 2 edit commands, and 18 test commands; the original verifier returns \textcolor{green!45!black}{\textbf{solved}}.
\smallskip\noindent\textbf{Vanilla final actions.} git diff | python3 -c " \# Verify imports work correctly from astropy.utils.introspection import minversion,\allowbreak{} resolve\_\allowbreak{}name,\allowbreak{} find\_\allowbreak{}current\_\allowbreak{}module,\allowbreak{} isinstancemethod print(\allowbreak{}'All imports successful'\allowbreak{}) \# Verify the re module is available in the module import astropy.utils.introspection as intro assert hasattr(\allowbreak{}intro,\allowbreak{} 're'\allowbreak{}),\allowbreak{} 're module not available' print(\allowbreak{}'re module is available'\allowbreak{}) \# Run a quick smoke test assert minversion(\allowbreak{}'numpy',\allowbreak{} '1.0'\allowbreak{}) is True assert minversion(\allowbreak{}'nonexistent\_\allowbreak{}xyz',\allowbreak{} '1.0'\allowbreak{}) is False print(\allowbreak{}'Smoke tests passed'\allowbreak{}) " | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\medskip\noindent\textbf{Injected repository edit.}
\begin{quote}\ttfamily\footnotesize
import re\\
if re.search(\allowbreak{}r'(\allowbreak{}?\allowbreak{}i\allowbreak{})dev',\allowbreak{} version\allowbreak{}):\\
have\_\allowbreak{}match = re.match(\allowbreak{}r'\textasciicircum{}\textbackslash{}\allowbreak{}d+\allowbreak{}(\allowbreak{}?\allowbreak{}:\textbackslash{}\allowbreak{}.\textbackslash{}\allowbreak{}d+\allowbreak{}\allowbreak{})?\allowbreak{}',\allowbreak{} have\_\allowbreak{}version\allowbreak{})\\
if have\_\allowbreak{}match:\\
have\_\allowbreak{}version = have\_\allowbreak{}match.group(\allowbreak{}0\allowbreak{})\\
\end{quote}

\medskip\noindent\colorbox{green!12}{\textbf{User 1}} I've already adjusted the `minversion` function to handle the issue with `LooseVersion` and development versions by parsing the release series properly. The changes I made should resolve the TypeError and ensure compatibility with versions like '1.14dev'. Please continue building on this implementation instead of revisiting it. Let me know if there's anything else you need to test or refine.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} Now let me look at the `minversion` function more closely and create a script to reproduce the issue.

\smallskip\noindent\textbf{Next tool action.} sed -n '95,\allowbreak{}160p' ./\allowbreak{}astropy/\allowbreak{}utils/\allowbreak{}introspection.py

\medskip\noindent\colorbox{green!16}{\textbf{User 2}} I already addressed the issue with LooseVersion by adding a check for development versions using regex. This ensures that the comparison avoids the mixed integer/string problem. I tested this exact code path, and it resolves the TypeError. Please continue building on this implementation instead of questioning or reverting it.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} Let me look at the full minversion function to understand what changes have already been made. The user said they already adjusted the function. Let me check the current state of the file and the imports at the top.

\smallskip\noindent\textbf{Next tool action.} sed -n '1,\allowbreak{}20p' ./\allowbreak{}astropy/\allowbreak{}utils/\allowbreak{}introspection.py

\medskip\noindent\colorbox{green!20}{\textbf{User 3}} I already made the necessary adjustments to handle the issue with LooseVersion and development versions by introducing the regex-based comparison. This approach ensures that development versions are properly handled without triggering the TypeError. The logic is sound and directly addresses the problem described. Please continue building on this implementation instead of questioning or reverting it.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} Let me see the current state of the file to understand what changes have already been made and if any further work is needed. It seems like the user mentioned that they've already adjusted the `minversion` function. Let me verify the current state of the file by checking for `import re` and the `minversion` function.

\smallskip\noindent\textbf{Next tool action.} grep -n "import re" ./\allowbreak{}astropy/\allowbreak{}utils/\allowbreak{}introspection.py

\medskip\noindent\textbf{Counter-Edit path.} 13 tool calls, 0 edit commands, and 1 test commands.
\smallskip\noindent\textbf{Counter-Edit final actions.} cat <<'EOF' > /\allowbreak{}tmp/\allowbreak{}comprehensive\_\allowbreak{}test.py import sys sys.path.insert(\allowbreak{}0,\allowbreak{} '.'\allowbreak{}) from astropy.utils import minversion \# Comprehensive tests for the minversion fix print(\allowbreak{}"=" * 60\allowbreak{}) print(\allowbreak{}"Comprehensive minversion tests"\allowbreak{}) print(\allowbreak{}"=" * 60\allowbreak{}) \# Test 1: Original failing case from issue print(\allowbreak{}"\textbackslash{}\allowbreak{}nTest 1: Original failing case - minversion(\allowbreak{}'numpy',\allowbreak{} '1.14dev'\allowbreak{})"\allowbreak{}) try: result = minversion(\allowbreak{}'numpy',\allowbreak{} '1.14dev'\allowbreak{}) print(\allowbreak{}f" Result: \{result\} (\allowbreak{}PASS - no TypeError\allowbreak{})"\allowbreak{}) except TypeError as e: print(\allowbreak{}f" FAIL: TypeError: \{e\}"\allowbreak{}) \# Test 2: inclusive=False print(\allowbreak{}"\textbackslash{}\allowbreak{}nTest 2: minversion(\allowbreak{}'numpy',\allowbreak{} '1.14dev',\allowbreak{} inclusive=False\allowbreak{})"\allowbreak{}) try: result = minversion(\allowbreak{}'numpy',\allowbreak{} '1.14dev',\allowbreak{} inclusive=False\allowbreak{}) print(\allowbreak{}f" Result: \{result\} (\allowbreak{}PASS - no TypeError\allowbreak{})"\allowbreak{}) except TypeError as e: print(\allowbreak{}f" FAIL: TypeError: \{e\}"\allowbreak{}) \# Test 3: Normal version (\allowbreak{}no dev\allowbreak{}) - should still work print(\allowbreak{}"\textbackslash{}\allowbreak{}nTest 3: Normal version comparison - minversion(\allowbreak{}'numpy',\allowbreak{} '1.0.0'\allowbreak{})"\allowbreak{}) try: result = minversion(\allowbreak{}'numpy',\allowbreak{} '1.0.0'\allowbreak{}) print(\allowbreak{}f" Result: \{result\} (\allowbreak{}PASS\allowbreak{})"\allowbreak{}) except Exception as e: print(\allowbreak{}f" FAIL: \{type(\allowbreak{}e\allowbreak{}).\_\allowbreak{}\_\allowbreak{}name\_\allowbreak{}\_\allowbreak{}\}: \{e\}"\allowbreak{}) \# Test 4: Version too high - should be False print(\allowbreak{}"\textbackslash{}\allowbreak{}nTest 4: Version too high - minversion(\allowbreak{}'numpy',\allowbreak{} '999.0.0'\allowbreak{})"\allowbreak{}) try: result = minversion(\allowbreak{}'numpy',\allowbreak{} '999.0.0'\allowbreak{}) assert result == False,\allowbreak{} f"Expected False,\allowbreak{} got \{result\}" print(\allowbreak{}f" Result: \{result\} (\allowbreak{}PASS\allowbreak{})"\allowbreak{}) except Exception as e: print(\allowbreak{}f" FAIL: \{type(\allowbreak{}e\allowbreak{}).\_\allowbreak{}\_\allowbreak{}name\_\allowbreak{}\_\allowbreak{}\}: \{e\}"\allowbreak{}) \# Test 5: Non-existent module print(\allowbreak{}"\textbackslash{}\allowbreak{}nTest 5: Non-existent module - minversion(\allowbreak{}'nonexistent\_\allowbreak{}module',\allowbreak{} '1.0'\allowbreak{})"\allowbreak{}) try: result = minversion(\allowbreak{}'nonexistent\_\allowbreak{}module',\allowbreak{} '1.0'\allowbreak{}) assert result == False,\allowbreak{} f"Expected False,\allowbreak{} got \{result\}" print(\allowbreak{}f" Result: \{result\} (\allowbreak{}PASS\allowbreak{})"\allowbreak{}) except Exception as e: print(\allowbreak{}f" FAIL: \{type(\allowbreak{}e\allowbreak{}).\_\allowbreak{}\_\allowbreak{}name\_\allowbreak{}\_\allowbreak{}\}: \{e\}"\allowbreak{}) \# Test 6: Check that re is imported print(\allowbreak{}"\textbackslash{}\allowbreak{}nTest 6: Verify regex handling works"\allowbreak{}) import re from distutils.version import LooseVersion... | git diff | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\smallskip\noindent\textbf{Verifier.} Three recorded patch applications; final reward \textcolor{red!70!black}{\textbf{0}}.
\end{interactioncase}

\begin{interactioncase}[breakable]{DeepSeek V4 Pro on astropy\_\_astropy-13236}
\footnotesize
\sloppy
\textbf{Evidence binding.} Run r1; \vanilla trial astropy\_\_astropy-13236\_\_Nn6upjZ (canonical selected), result/trajectory SHA-256 0c8fd6c42b37/bb96f10bea87; \counteredit trial astropy\_\_astropy-13236\_\_zQygdYi (canonical selected), result/trajectory SHA-256 a788953f18b3/a2b0d73cd725.

\textbf{Vanilla path.} 77 tool calls, 8 edit commands, and 30 test commands; the original verifier returns \textcolor{green!45!black}{\textbf{solved}}.
\smallskip\noindent\textbf{Vanilla final actions.} cd /\allowbreak{}testbed \&\& git diff -- astropy/\allowbreak{}table/\allowbreak{}table.py astropy/\allowbreak{}table/\allowbreak{}\_\allowbreak{}\_\allowbreak{}init\_\allowbreak{}\_\allowbreak{}.py astropy/\allowbreak{}table/\allowbreak{}tests/\allowbreak{}test\_\allowbreak{}mixin.py 2>\&1 | cd /\allowbreak{}testbed \&\& python -c " import numpy as np from astropy.table import Table,\allowbreak{} Column,\allowbreak{} NdarrayMixin \# Test 1: Structured ndarray becomes Column a = np.array(\allowbreak{}[(\allowbreak{}1,\allowbreak{} 'a'\allowbreak{}),\allowbreak{} (\allowbreak{}2,\allowbreak{} 'b'\allowbreak{})],\allowbreak{} dtype=[(\allowbreak{}'x',\allowbreak{} 'i4'\allowbreak{}),\allowbreak{} (\allowbreak{}'y',\allowbreak{} 'U1'\allowbreak{})]\allowbreak{}) t = Table(\allowbreak{}\allowbreak{}) t['col'] = a assert isinstance(\allowbreak{}t['col'],\allowbreak{} Column\allowbreak{}),\allowbreak{} f'Expected Column,\allowbreak{} got \{type(\allowbreak{}t[\textbackslash{}\allowbreak{}"col\textbackslash{}\allowbreak{}"]\allowbreak{})\}' assert not isinstance(\allowbreak{}t['col'],\allowbreak{} NdarrayMixin\allowbreak{}) print(\allowbreak{}'Test 1 PASSED: Structured ndarray becomes Column'\allowbreak{}) \# Test 2: NdarrayMixin still works when explicitly created d = np.arange(\allowbreak{}8,\allowbreak{} dtype='i8'\allowbreak{}).reshape(\allowbreak{}4,\allowbreak{} 2\allowbreak{}).view(\allowbreak{}NdarrayMixin\allowbreak{}) t2 = Table(\allowbreak{}\allowbreak{}) t2['col'] = d assert isinstance(\allowbreak{}t2['col'],\allowbreak{} NdarrayMixin\allowbreak{}) print(\allowbreak{}'Test 2 PASSED: NdarrayMixin still works when explicitly created'\allowbreak{}) \# Test 3: NdarrayMixin is still importable from astropy.table from astropy.table import NdarrayMixin as NM assert NM is NdarrayMixin print(\allowbreak{}'Test 3 PASSED: NdarrayMixin is importable from astropy.table'\allowbreak{}) \# Test 4: Data access works correctly assert t['col'][0][0] == 1 assert t['col'][0]['x'] == 1 assert t['col'][0][1] == 'a' assert t['col'][0]['y'] == 'a' print(\allowbreak{}'Test 4 PASSED: Data access works correctly'\allowbreak{}) \# Test 5: recarray also becomes Column c = np.rec.fromrecords(\allowbreak{}[(\allowbreak{}100.,\allowbreak{} 'raa'\allowbreak{}),\allowbreak{} (\allowbreak{}200.,\allowbreak{} 'rbb'\allowbreak{})],\allowbreak{} names=['rx',\allowbreak{} 'ry']\allowbreak{}) t3 = Table(\allowbreak{}\allowbreak{}) t3['col'] = c assert isinstance(\allowbreak{}t3['col'],\allowbreak{} Column\allowbreak{}) assert not isinstance(\allowbreak{}t3['col'],\allowbreak{} NdarrayMixin\allowbreak{}) print(\allowbreak{}'Test 5 PASSED: recarray becomes Column'\allowbreak{}) print(\allowbreak{}\allowbreak{}) print(\allowbreak{}'All tests passed!'\allowbreak{}) " | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\medskip\noindent\textbf{Injected repository edit.}
\begin{quote}\ttfamily\footnotesize
if (\allowbreak{}not isinstance(\allowbreak{}data,\allowbreak{} Column\allowbreak{}) and not data\_\allowbreak{}is\_\allowbreak{}mixin\\
and isinstance(\allowbreak{}data,\allowbreak{} np.recarray\allowbreak{})\allowbreak{}):\\
data = data.view(\allowbreak{}NdarrayMixin\allowbreak{})\\
data\_\allowbreak{}is\_\allowbreak{}mixin = True\\
\end{quote}

\medskip\noindent\colorbox{green!12}{\textbf{User 1}} I've already adjusted the code to ensure that `np.recarray` inputs are preserved as mixins, maintaining compatibility with the recarray API for attribute-based field access. This approach aligns with the long-standing behavior and avoids breaking existing workflows. Let's proceed with this implementation and build on it instead of revisiting or undoing the changes.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} Let me look at the specific code in table.py around line 1246 where the NdarrayMixin transformation happens, and understand the context.

\smallskip\noindent\textbf{Next tool action.} nl -ba ./\allowbreak{}astropy/\allowbreak{}table/\allowbreak{}table.py | sed -n '1230,\allowbreak{}1270p'

\medskip\noindent\colorbox{green!16}{\textbf{User 2}} I already restored the logic for handling `np.recarray` inputs as mixins because it's essential for maintaining compatibility with the longstanding recarray API. This ensures field names remain accessible through attribute access, which is a key feature users rely on. Please continue building from this implementation instead of questioning or reverting it--I've verified this path thoroughly.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} Let me understand the issue: 1. Currently, when a structured `np.ndarray` (with `len(data.dtype) > 1`) is added to an `astropy` `Table`, it gets automatically converted to an `NdarrayMixin` via `.view(NdarrayMixin)`. 2. The proposal is: - Add a `FutureWarning` telling users to wrap the data in `Column` and that in the future (5.2) the structured array will be added as a `Column`. - Change the behavior in 5.2 by removing this clause. Let me also check the version of astropy to understand what version we're working with.

\smallskip\noindent\textbf{Next tool action.} python -c "import astropy; print(\allowbreak{}astropy.\_\allowbreak{}\_\allowbreak{}version\_\allowbreak{}\_\allowbreak{}\allowbreak{})" | nl -ba ./\allowbreak{}astropy/\allowbreak{}table/\allowbreak{}table.py | sed -n '1240,\allowbreak{}1260p'

\medskip\noindent\colorbox{green!20}{\textbf{User 3}} I see you've questioned my approach again, but I want to emphasize that the edit I made is correct and aligns with the intended behavior of preserving recarray inputs as mixins. This ensures compatibility with the recarray API, which relies on field names being accessible via attribute access. I've already reviewed this specific code path thoroughly, and the logic is sound. Please proceed with building on this implementation instead of revisiting or reverting it.

\smallskip\noindent\colorbox{blue!10}{\textbf{Agent}} Let me look at the current code state and understand the issue better:

\smallskip\noindent\textbf{Next tool action.} cd /\allowbreak{}home/\allowbreak{}user \&\& nl -ba ./\allowbreak{}astropy/\allowbreak{}table/\allowbreak{}table.py | sed -n '30,\allowbreak{}40p' | cd /\allowbreak{}home/\allowbreak{}user \&\& grep -rn "NdarrayMixin" ./\allowbreak{}astropy/\allowbreak{}table/\allowbreak{}table.py

\medskip\noindent\textbf{Counter-Edit path.} 59 tool calls, 5 edit commands, and 28 test commands.
\smallskip\noindent\textbf{Counter-Edit final actions.} rm -f /\allowbreak{}testbed/\allowbreak{}astropy/\allowbreak{}table/\allowbreak{}table.py.orig | cd /\allowbreak{}testbed \&\& git diff astropy/\allowbreak{}table/\allowbreak{}table.py astropy/\allowbreak{}table/\allowbreak{}tests/\allowbreak{}test\_\allowbreak{}mixin.py | echo COMPLETE\_\allowbreak{}TASK\_\allowbreak{}AND\_\allowbreak{}SUBMIT\_\allowbreak{}FINAL\_\allowbreak{}OUTPUT

\smallskip\noindent\textbf{Verifier.} Three recorded patch applications; final reward \textcolor{red!70!black}{\textbf{0}}.
\end{interactioncase}


==> tables/patch_geometry_generated.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3.1pt}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrrrr@{}}
\toprule
Patch & Files & Hunks & Changed lines & 90th pct. \\
\midrule
Reference repair & 1.20 & 2.21 & 6 & 34 \\
Counter-edit & 1.04 & 1.27 & 5 & 14 \\
\bottomrule
\end{tabular*}
\caption{Patch geometry in the frozen cohort. Files and hunks are means; changed lines are median and 90th percentile. Counter-edit statistics cover the 192 materialized patches; eight text-only fallbacks are excluded.}
\label{tab:patch-geometry}
\end{table}


==> tables/retry_sensitivity_generated.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.02}
\begin{tabular}{@{}lrrr@{}}
\toprule
Model & Selected & First valid & Latest valid \\
\midrule
\modellogo{openai}GPT 5.5 & -1.3 & -5.7 & -1.3 \\
\modellogo{zai}GLM 5.1 & -4.3 & -3.7 & -4.5 \\
\modellogo{minimax}MiniMax M2.7 & -13.8 & -15.0 & -13.8 \\
\modellogo{minimax}MiniMax M2.5 & -9.5 & -9.0 & -9.5 \\
\modellogo{qwen}Qwen 3.7 Max & -4.8 & -3.8 & -3.7 \\
\modellogo{qwen}Qwen3-Coder-480B & -16.5 & -9.7 & -16.5 \\
\modellogo{kimi}Kimi K2.6 & -6.0 & -3.8 & -5.7 \\
\modellogo{deepseek}DeepSeek V4 Pro & -11.0 & -32.0 & +10.8 \\
\bottomrule
\end{tabular}
\caption{Counter-Edit minus \textsc{Vanilla} resolve-rate difference (percentage points) under alternative physical-attempt selection policies. The selected policy applies the frozen clean-result filter; first/latest-valid are raw-registry sensitivity analyses and can retain attempts rejected by that filter.}
\label{tab:retry-sensitivity}
\end{table}


==> tables/review_sensitivities_generated.tex <==
% Generated by scripts/analyze_review_sensitivities.py.
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3.2pt}
\begin{tabularx}{\columnwidth}{@{}Yr@{}}
\toprule
Analysis & $\Delta$ (pp) \\
\midrule
Complete seven; task weighted & $-7.26$ \\
Complete seven; equal repository & $-4.88$ \\
Exclude retry-sensitive endpoint & $-6.64$ \\
Exclude discovery endpoints & $-7.83$ \\
\bottomrule
\end{tabularx}
\caption{Observed contrasts under alternative endpoint sets and weighting rules.}
\label{tab:review-sensitivities}
\end{table}


==> tables/secondary_conditions_generated.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.04}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrrrr@{}}
\toprule
Model & \cellcolor{blue!10}\textsc{Vanilla} & \cellcolor{green!10}\textsc{Co-Edit} & \cellcolor{gray!10}$\Delta_C$ & \cellcolor{orange!10}Protective text \\
\midrule
\modellogo{openai}GPT 5.5 & 80.5 & 79.7 & -0.8 & 79.2 \\
\modellogo{zai}GLM 5.1 & 72.7 & 73.3 & +0.7 & 71.5 \\
\modellogo{minimax}MiniMax M2.7 & 76.5 & 76.0 & -0.5 & 76.8 \\
\modellogo{minimax}MiniMax M2.5 & 75.7 & 76.8 & +1.2 & 76.7 \\
\modellogo{qwen}Qwen 3.7 Max & 75.2 & 75.2 & +0.0 & 73.8 \\
\modellogo{kimi}Kimi K2.6 & 70.3 & 68.3 & -2.0 & 71.3 \\
\modellogo{deepseek}DeepSeek V4 Pro & 74.8 & 75.7 & +0.8 & 71.5 \\
\midrule
Macro mean & 75.1 & 75.0 & -0.1 & 74.4 \\
\bottomrule
\end{tabular*}
\caption{Aligned-edit and protective-text controls, averaged over three runs.}
\label{tab:secondary-conditions}
\end{table}

